Mitigating Object and Action Hallucinations in Multimodal LLMs via Self-Augmented Contrastive Alignment

Recent advancement in multimodal LLMs (MLLMs) has demonstrated their remarkable capability to generate descriptive captions for input videos. However, these models suffer from factual inaccuracies in the generated descriptions, causing severe hallucination issues. While prior works have explored alleviating hallucinations for static images, jointly mitigating visual object and temporal action hallucinations for dynamic videos remains a challenging and unsolved task. To tackle this challenge, we propose a Self-Augmented Contrastive Alignment (SANTA) framework for enabling object and action faithfulness by exempting the spurious correlations and enforcing the emphasis on visual facts. SANTA employs a hallucinative self-augmentation scheme to identify the potential hallucinations that lie in the MLLM and transform the original captions to the contrasted negatives. Furthermore, we develop a tracklet-phrase contrastive alignment to match the regional objects and relation-guided actions with their corresponding visual and temporal phrases. Extensive experiments demonstrate that SANTA outperforms existing methods in alleviating object and action hallucinations, yielding superior performance on the hallucination examination benchmarks.

==> rebuttal_materials/ablate_vg.tex <==
\begin{table}[htbp]
\centering
\fontsize{8.5}{9.5}\selectfont
\setlength{\tabcolsep}{2mm}
\renewcommand{\arraystretch}{1.12}
\vspace{-3.5mm}
\caption{\textbf{Ablation of~\textit{SANTA} w/ the quality of object tracklets.}}
\vspace{-3mm}
\label{tab:rebuttal:ablate_vg}
\resizebox{\linewidth}{!}{%
\begin{tabular}{lcccc}
\toprule
\multirow{2}{*}{\textbf{Method}}
    & \multicolumn{2}{c}{\textbf{HalFscore \ib{[4]}}}
    & \multicolumn{2}{c}{\textbf{weighted-HalFscore}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
    & {\footnotesize \textbf{\shortstack{Avg. F1$_\text{Obj}$↑}}}
    & {\footnotesize \textbf{\shortstack{Avg. F1$_\text{Act}$↑}}}
    & {\footnotesize \textbf{\shortstack{Avg. F1$_\text{Obj}$↑}}}
    & {\footnotesize \textbf{\shortstack{Avg. F1$_\text{Act}$↑}}} \\
\midrule
HACL \ib{[12]}
    & 36.5 & 28.5 & 52.8 & 30.5 \\
SANTA w/ G-SAM2 ($t$=0.15)   
    & 37.2 & 29.4 & 54.0 & 31.6 \\
SANTA w/ G-SAM2 ($t$=0.25)
    & \textbf{37.9} & \textbf{30.0} & \textbf{54.8} & \textbf{32.7} \\
\bottomrule
\end{tabular}
}
\vspace{-4.5mm}
\end{table}


==> rebuttal_materials/videomme.tex <==
\begin{table}[htbp]
    \centering
    \vspace{-2mm}
    \caption{\textbf{Evaluations on the VideoMME \ib{[8]}. Subcolumns \textbf{w/} and \textbf{w/o} denote whether subtitles are used.}}
    \label{tab:rebuttal:videomme}
    \vspace{-3.5mm}
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{l *{4}{cc}}
        \toprule
        \multirow{2}{*}{\textbf{Method}} 
            & \multicolumn{2}{c}{\textbf{Short}} 
            & \multicolumn{2}{c}{\textbf{Medium}} 
            & \multicolumn{2}{c}{\textbf{Long}} 
            & \multicolumn{2}{c}{\textbf{Overall}} \\
        \cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
            & \textbf{w/} & \textbf{w/o} 
            & \textbf{w/} & \textbf{w/o} 
            & \textbf{w/} & \textbf{w/o} 
            & \textbf{w/} & \textbf{w/o} \\
        \midrule
        LLaVA-Video \ib{[37]} 
            & \textcolor{gray}{80.1} & \textcolor{gray}{77.0}
            & \textcolor{gray}{66.6} & \textcolor{gray}{61.8}
            & \textcolor{gray}{58.3} & \textcolor{gray}{52.1}
            & \textcolor{gray}{68.3} & \textcolor{gray}{63.6} \\
        \cmidrule{2-9}
        +SFT \ib{[37]} 
            & 54.8 & 56.8 
            & 45.4 & 45.9 
            & 35.3 & 35.0 
            & 45.2 & 45.9 \\
        +HACL \ib{[12]} 
            & 73.1 & 69.9 
            & 62.3 & 57.9 
            & 53.2 & 51.4 
            & 62.9 & 59.7 \\
        +SANTA (Ours) 
            & \textbf{76.8} & \textbf{72.3} 
            & \textbf{64.6} & \textbf{59.8} 
            & \textbf{55.4} & \textbf{49.6} 
            & \textbf{65.6} & \textbf{60.6} \\
        \bottomrule
    \end{tabular}
    }
    \vspace{-5.5mm}
\end{table}


==> tables/dream1k_overall_only.tex <==
\begin{wraptable}{R}{0.3\textwidth}
    \centering
    \caption{Quantitative comparison of hallucination mitigation methods on the Dream1k~\cite{dream1k} benchmark (Overall).}
    \label{tab:dream1k_overall}
    \vspace{1mm}
    \begin{tabular}{l c}
        \toprule
        \textbf{Method} & \textbf{Overall} \\
        \midrule
        LLaVA-Video~\cite{llavavideo}  & \textcolor{gray}{32.5} \\
        +SFT~\cite{llavavideo}         & 29.2 \\
        +HALVA~\cite{halva}            & 32.6 \\
        +HACL~\cite{hacl}              & 30.7 \\
        +SANTA (Ours)                  & \textbf{32.7} \\
        \bottomrule
    \end{tabular}
    \vspace{-2mm}
\end{wraptable}


==> tables/factvc.tex <==
\begin{table*}[ht]
\centering
\caption{Performance Comparison on FactVC}
\resizebox{0.8\textwidth}{!}{% 調整表格大小以適應頁面寬度
\begin{tabular}{l|c|c|c}
\toprule
\textbf{Exp. Name} & \textbf{$\text{FactVC}_{\text{prec.}}$ ($\uparrow$)} & \textbf{$\text{FactVC}_{\text{rec.}}$ ($\uparrow$)} & \textbf{$\text{FactVC}_{\text{f1.}}$ ($\uparrow$)} \\
\midrule
LLaVA-Video~\cite{llavavideo} & 36.4 & 39.9 & 37.9 \\
LLaVA-Video+SFT~\cite{llavavideo} & 38.2 & 41.7 & 39.7 \\
LLaVA-Video+DeCo~\cite{deco} & - & - & - \\
LLaVA-Video+HACL~\cite{hacl} & - & - & - \\
LLaVA-Video+HALVA~\cite{halva} & - & - & - \\
LLaVA-Video+SANTA (Ours) & \textbf{39.4} & \textbf{42.9} & \textbf{40.9} \\
\bottomrule
\end{tabular}}
\label{tab:factvc}
\end{table*}

==> tables/miradata_halfscore.tex <==
\begin{table*}[t]
\centering
\vspace{-5mm}
\caption{Evaluation on both object and action hallucinations 
with the metrics proposed by HalFscore~\cite{perturbollava} on MiraData-9k~\cite{mirabench} across three types of video captions: overall content, main object, and background details. \textbf{Bold} and \underline{underline} indicate the best and second best results, respectively.}
\vspace{-2mm}

\resizebox{1.0\linewidth}{!}{%
\begin{tabular}{l|>{\centering\arraybackslash}m{2.1cm}|>{\centering\arraybackslash}m{2.1cm}|>{\centering\arraybackslash}m{2.1cm}|>{\centering\arraybackslash}m{2.1cm}|>{\centering\arraybackslash}m{2.1cm}|>{\centering\arraybackslash}m{2.1cm}}
\toprule
\textbf{Method} & \textbf{HalFscore$_\text{Hallu.}$-Act (↓)} & \textbf{HalFscore$_\text{Hallu.}$-Obj (↓)} 
               & \textbf{HalFscore$_\text{cover.}$-Act (↑)} & \textbf{HalFscore$_\text{cover.}$-Obj (↑)}
               & \textbf{HalFscore$_\text{F1}$-Act (↑)}    & \textbf{HalFscore$_\text{F1}$-Obj (↑)}  \\
\midrule
\multicolumn{7}{c}{\textcolor{gray}{Overall Content Captioning}} \\
LLaVA-Video~\cite{llavavideo}       & 76.5& 79.4& \textbf{33.0}& 52.1& 27.7& 29.5\\
\quad+HACL~\cite{hacl}        & \textbf{65.2}& \textbf{70}& 29.9& 53.7& 32.2& 38.4\\
\quad+\textbf{SANTA (Ours)}   & \underline{65.3}& \underline{70.1}& \underline{32.0}& \textbf{56.6}& \cellcolor{cyan!25}\textbf{33.3}& \cellcolor{cyan!25}\textbf{38.9}\\
\midrule
\multicolumn{7}{c}{\textcolor{gray}{Main Object Captioning}} \\
LLaVA-Video~\cite{llavavideo}       & 75.5& 83.1& 23.8& 43.1& 24.1& 24.3\\
\quad+HACL~\cite{hacl}        & 67.9& 79.4& 26.3& 52.3& 28.9& 29.6\\
\quad+\textbf{SANTA (Ours)}   & \textbf{65.2}& \textbf{77.8}& \textbf{26.8}& \textbf{53.1}& \cellcolor{cyan!25}\textbf{30.3}& \cellcolor{cyan!25}\textbf{31.4}\\
\midrule
\multicolumn{7}{c}{\textcolor{gray}{Background Captioning}} \\
LLaVA-Video~\cite{llavavideo}       & 85.4& 78.7& 19.4& 42.3& 16.7& 28.4\\
\quad+HACL~\cite{hacl}        & \textbf{65.7}& \textbf{60.3}& 18.8& 43.5& 24.3& 41.5\\
\quad+\textbf{SANTA (Ours)}   & \underline{66.5}& \underline{61.4}& \textbf{21.1}& \textbf{45.9}& \cellcolor{cyan!25}\textbf{25.9}& \cellcolor{cyan!25}\textbf{41.9}\\
\bottomrule
\end{tabular}
}
\label{tab:miradata_halfscore}
\end{table*}


==> tables/videomme_and_dream1k.tex <==
\begin{table*}[t]
    \centering
    \caption{Quantitative comparisons with hallucination mitigation methods on general video question answering and captioning benchmarks.}
    \label{tab:videomme_dream1k}
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{l *{8}{c} *{6}{c}}
        \toprule
        \multirow{3}{*}{\textbf{Method}} 
            & \multicolumn{8}{c}{\textbf{VideoMME}} 
            & \multicolumn{6}{c}{\textbf{Dream1k}} \\
        \cmidrule(lr){2-9} \cmidrule(lr){10-15}
            & \multicolumn{4}{c}{\textbf{with subtitles}} 
            & \multicolumn{4}{c}{\textbf{without subtitles}} 
            % Dream1k這層不填內容，讓下一層multirow標題置中
            & \multicolumn{1}{c}{} 
            & \multicolumn{1}{c}{} 
            & \multicolumn{1}{c}{} 
            & \multicolumn{1}{c}{} 
            & \multicolumn{1}{c}{} 
            & \multicolumn{1}{c}{} \\
        \cmidrule(lr){2-5} \cmidrule(lr){6-9}
            & \textbf{Short} & \textbf{Medium} & \textbf{Long} & \textbf{Overall}
            & \textbf{Short} & \textbf{Medium} & \textbf{Long} & \textbf{Overall}
            % Dream1k這層才寫multirow（跨2層置中）
            & \multirow{-2}{*}{\textbf{\shortstack{Animation}}}
            & \multirow{-2}{*}{\textbf{\shortstack{Live\\action}}}
            & \multirow{-2}{*}{\textbf{Short}}
            & \multirow{-2}{*}{\textbf{Stock}}
            & \multirow{-2}{*}{\textbf{Youtube}}
            & \multirow{-2}{*}{\textbf{Overall}} \\
        \midrule
        LLaVA-Video~\cite{llavavideo} & 78.7 & 65.6 & 56.1 & 66.7 & 74.7 & 61.8 & 49.9 & 62.1 & 27.6 & 31.4 & 33.4 & 36.7 & 33.0 & 32.5 \\
        +SFT~\cite{llavavideo}   & 54.8 & 45.4 & 35.3 & 45.2 & 56.8 & 45.9 & 35.0 & 45.9 & 19.9 & 27.7 & 28.3 & 36.0 & 33.0 & 29.2 \\
        +HALVA~\cite{halva}      & 80.3 & 66.3 & 57.2 & 68.0 & 76.3 & 62.2 & 52.1 & 63.6 & 26.2 & 32.3 & 34.6 & 38.2 & 31.8 & 32.6 \\
        +HACL~\cite{hacl}        & 73.1 & 62.3 & 53.2 & 62.9 & 69.9 & 57.9 & 51.4 & 59.7 & 23.9 & 28.1 & 30.0 & 37.5 & 33.2 & 30.7 \\
        +SANTA (Ours)            & 76.8 & 64.6 & 55.4 & 65.6 & 72.3 & 59.8 & 49.6 & 60.6 & 24.7 & 31.0 & 31.8 & 41.2 & 33.4 & 32.7 \\
        \bottomrule
    \end{tabular}
    }
\end{table*}


==> tables/vidhal_all.tex <==
% \begin{table*}[ht]
% \centering
% \caption{Performance Comparison on VidHal}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{l|c|c|c||c|c|c||c}
% \toprule
% \textbf{Exp. Name} & \textbf{Action-Acc. ($\uparrow$)} & \textbf{Object-Acc. ($\uparrow$)} & \textbf{Attribute-Acc. ($\uparrow$)} & \textbf{Direction-Acc. ($\uparrow$)} & \textbf{Order-Acc. ($\uparrow$)} } \\
% \midrule
% LLaVA-Video~\cite{llavavideo}     & 83.1 & 84.3 & 63.4 & 34.8 & 66.2 
% LLaVA-Video+SFT~\cite{llavavideo} & 65.6 & 36.3 & 40.0 & 35.3 & 36.8 \\
% LLaVA-Video+DeCo~\cite{deco} & 84.7 & 82.8 & 63.4 & 33.3 & 68.6 \\
% LLaVA-Video+HACL~\cite{hacl} & - & - & - & - & -  \\
% LLaVA-Video+HALVA~\cite{halva} & - & - & - & - & - \\
% LLaVA-Video+SANTA (ours) & \textbf{85.8} & \textbf{86.3} & 63.4 & \textbf{45.1} & 51.5\\
% \bottomrule
% \end{tabular}}
% \label{tab:performance_comparison}
% \end{table*}
